The Case for the Anonymization of Offloaded Computation

Computation offloading (often to external computing resources over a network) has become a necessity for modern applications. At the same time, the proliferation of machine learning techniques has empowered malicious actors to use such techniques in order to breach the privacy of the execution process for offloaded computations. This can enable malicious actors to identify offloaded computations and infer their nature based on computation characteristics that they may have access to even if they do not have direct access to the computation code. In this paper, we first demonstrate that even non-sophisticated machine learning algorithms can accurately identify offloaded computations. We then explore the design space of anonymizing offloaded computations through the realization of a framework, called Camouflage. Camouflage features practical mechanisms to conceal characteristics related to the execution of computations, which can be used by malicious actors to identify computations and orchestrate further attacks based on identified computations. Our evaluation demonstrated that Camouflage can impede the ability of malicious actors to identify executed computations by up to 60%, while incurring modest overheads for the anonymization of computations.

==> sections/eval.tex <==
\section {Evaluation}
\label{sec:eval}

In this section, we first present our evaluation setup and we then discuss our evaluation results.

%We evaluate our proposed idea for computation anonymization in four categories. Firstly, we evaluate introducing fake nodes to computation graphs with our own synthetic dataset, then to confirm our findings are relevant for real-world scenarios we run the fake node generation idea with the data from Alibaba Cluster Dataset [refer]. Next, we follow our mix & match approach over our synthetic model and the Alibaba Cluster Dataset. \newline

\subsection {Evaluation Setup}

We implement a prototype of \sol which supports three modes (the \solOne, \mix, and \hybrid modes) to evaluate its performance and design tradeoffs. We use a Decision Tree \cite{quinlan1987simplifying}, a k-Nearest Neighbors (kNN) \cite{altman1992introduction}, and a Neural Network (NN) \cite{dayhoff1990neural} models as the attack models to identify executed computations. Figure \ref{Figure:eval_steps} shows the process we followed to evaluate \sol. We utilize three computation datasets to train the attack models: a synthetic dataset, an ML/AL dataset, and a real-world data from Alibaba cloud \cite{alibaba}. We summarize the characteristics of these datasets in Table~\ref{Table:datasets} and we discuss them further below. 

Once an attack model is trained, we measure and use the accuracy of the trained model as our baseline (\ie case of no anonymization) to quantify the effectiveness of \sol. Subsequently, \sol (either the \solOne mode or the \mix mode or the \hybrid mode) is applied to a computation to anonymize it, the anonymized computation graph is executed, and its features are collected. The collected features are fed to the trained attack model to predict the identity of the computation and we again measure the accuracy of the model for anonymized computations. Finally, we compare the accuracy of the attack model measured before and after the anonymization. The reduction in accuracy indicates the effectiveness of \sol. We also measure the time required by \sol to convert an original graph to the corresponding anonymized graph and the overhead (in terms of time, and CPU usage) introduced to the execution process because of anonymization.

%\textcolor{red}{table about the machine, describe metrics}
%\textcolor{red}{add a figure to show the steps of the how we evaluate --- 1) generate(collect) the dataset, 2) trained the attack model (3) used \sol to anonymize each graph 4) Compared the accuracy of the attack model before and after the anonymization. }

\begin{figure}[!t]
%\vspace{-0.2cm}
 \centering
 \includegraphics[width=1\columnwidth]{figs/eval_steps.pdf}
 \vspace{-0.5cm}
 \caption{An overview of the \sol evaluation process.} 
 \label{Figure:eval_steps}
 \vspace{-0.2cm}
\end{figure}

%\textcolor{red}{Talk about the evaluation setup: mention that we have implemented a prototype of \sol, we evaluated it based on two datasets, that we use different machine learning models to verify the validity of our experiments, how we trained and validated these models.}

\begin{table*}[t]
\centering
\caption{Datasets used for the evaluation of \sol and their characteristics.}
\resizebox{1\textwidth}{!}{%
\label{Table:datasets}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Dataset}      & \textbf{Features}                                                               & \textbf{Nature}             & \textbf{\begin{tabular}[c]{@{}c@{}}Average Number \\ of Nodes\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Average Node \\ Degree\end{tabular}} \\ \hline
Synthetic dataset   & \begin{tabular}[c]{@{}c@{}}CPU usage, memory\\ usage, completion time,\\ inputs/outputs\end{tabular} & \begin{tabular}[c]{@{}c@{}} Computation graphs are formed \\ by interconnecting nodes that \\ represent popular algorithmic \\ operations (sorting, searching, hashing, \\ encryption, decryption, compression, \\ decompression). \end{tabular}                       & 3.9                                                              & 3.0                                                          \\ \hline
%std: 1.7 & 0.77


\begin{tabular}[c]{@{}c@{}} ML/AI graph dataset \end{tabular}   & \begin{tabular}[c]{@{}c@{}} CPU and memory usage, \\ input and output sizes, \\ completion times \end{tabular}    & \begin{tabular}[c]{@{}c@{}} Image processing, image and text \\classification graphs, language \\ translation model graphs,\\ automatic image annotation, etc. \end{tabular}  & 6.4                                                                             &     2.15                                                                    \\ \hline

Alibaba Cloud dataset  &\begin{tabular}[c]{@{}c@{}} CPU and memory \\ usage (normalized), \\ completion times \end{tabular}                                                                                  & Data-center cluster dataset & 1.72                                                                             &     2.0                                                                    \\ \hline


\end{tabular}


%\end{tabular}

}


\end{table*}

\noindent\textbf{Synthetic dataset:} %We used ten different realistic computation graphs to create the synthetic dataset for our experiments. To create these graphs realistic, we use popular operations such as sorting, searching, hashing, encryption, decryption, compression, decompression, etc. as the nodes of each graph, and combine multiple nodes in a logical way. For instance, if a user offloads an encrypted query, then the graph  decrypts the query, searches match for the query, and encrypts the search results to respond in a sequential way. 
This dataset includes computation graphs, which are formed by interconnecting nodes that represent popular algorithmic operations (sorting, searching, hashing, encryption, decryption, compression, decompression).
We divided the computations of this dataset into two categories: delay-sensitive and delay-tolerant computations. For our evaluation, we considered delay-sensitive computations as more important than delay-tolerant computations (\ie delay-sensitive computations need to be executed as quickly as possible). The dataset contains the number of inputs and the outputs, the input and output sizes, the completion time of each computation.

%\textcolor{red}{maybe one or two example figures of the graphs}
%\textcolor{red}{Describe the synthetic dataset}

\noindent\textbf{ML/AI graph dataset:} For our evaluation, we took a number of ``off-the-shelf" widely used real-world machine learning and artificial intelligence graphs as described in Table \ref{Table:datasets},  and ran them with different hyper-parameters and training dataset sizes to collect features of these workloads. We selected graphs mainly related to different ML/AI use cases because large DAG nature of these graphs and a wide range of real-word use cases and services related to ML/AI provided by commercial cloud providers such as Amazon SageMaker, Azure Applied AI Services, Azure Machine Learning, Vertex AI by Google Cloud, etc.  


\noindent\textbf{Alibaba cloud dataset:} This dataset contains different pieces of information collected from 4000 machines over a period of eight days. Although the dataset comes with information on servers, containers, and batch jobs, we utilize the data related to the batch job to evaluate the performance of \sol as our main goal is to identify what types of computations are being executed. A job (\ie a computation graph) is a set of tasks (\ie nodes) that are dependent on each other forming a DAG. The jobs are categorized into multiple types that we intend to identify with our attack models.
%We categorize the jobs into multiple classes based on tasks within a job (\ie similarity among the jobs) since multiple jobs may have the same tasks but the number of instances of each task can vary from one job to another job although both jobs perform the same type of computation, and list all the information for each type of job. 
The dataset provides CPU and memory usage in a normalized format, as well as completion times.

%\textcolor{red}{verify again}
%\textcolor{red}{Describe the alibaba dataset} 

\noindent\textbf{Evaluation metrics:} We use two metrics to evaluate \sol: (i) the attack model's identification accuracy; and (ii) the overhead introduced due to anonymization. The reduction of the attack model's accuracy with respect to the baseline model (\ie no anonymization) indicates the effectiveness of \sol. We quantify overhead as the additional time and computing resources (CPU and memory usage) needed to complete an anonymized computation as compared to the original computation with no anonymization.

%\textcolor{red}{just time overhead? anything else... like memory, cpu. Also should normalize the overhead as percentage?}

\subsection {Evaluation Results}
\label{subsec:results}

We present our evaluation results for all three operation modes of \sol below. 

\subsubsection{\solOne mode}

\noindent\textbf{\newline Effect of anonymization on accuracy:} In Figure \ref{figure:solOne_acc_level}, we present the computation identification accuracy results for different attack models when computations are anonymized through the \solOne mode. For all three datasets, each attack model demonstrates a similar trend. Specifically, the computation identification accuracy of all three models decreases as the anonymization level increases. \solOne is able to achieve up to 60\% accuracy reduction. But as we increase the anonymization level, the effectiveness of \solOne (\ie the reduction of accuracy) becomes smaller, since the \solOne mode adds adequate randomness to the original computation graph. As a result, the models cannot find enough useful patterns among the features to correlate with computations. The results also show that the models have relatively better accuracy for the synthetic dataset and the ML/AL dataset at any given anonymization level than the Alibaba cloud dataset, since the Alibaba cloud dataset contains fewer features (\eg no input and output data sizes) that can be used for the identification of computation compared to other two datasets. 


\begin{figure*}[!th]
\vspace{-0.1cm}
\captionsetup[subfigure]{aboveskip=-0.00000000000000001pt,belowskip=-0.00000000000000001pt}
	\centering
	\begin{subfigure}{0.33\textwidth}
		\centering
		\includegraphics[scale=0.22]{figs/solOne_syn_acc_level.pdf}
		\caption{Synthetic dataset.}
		\label{Figure:solOne_syn_acc_level}
	\end{subfigure} \hfil
	%\vspace{0.2cm}
	\begin{subfigure}{0.33\textwidth}
	    \centering
	    \includegraphics[scale=0.22]{figs/solOne_ml_acc_level.pdf}
	    \caption{ML/AI dataset}
	    \label{Figure:solOne_ml_acc_level}
	\end{subfigure}\hfil
	\begin{subfigure}{0.33\textwidth}
	    \centering
	    \includegraphics[scale=0.22]{figs/solOne_alibaba_acc_level.pdf}
	    \caption{Alibaba cloud dataset.}
	    \label{Figure:alibaba_syn_acc_level}
	\end{subfigure}\hfil
	\vspace{-0.3cm}
	\caption{Identification accuracy of different attack models for different anonymization levels using \solOne mode.}
	\label{figure:solOne_acc_level}
	\vspace{-0.2cm}
\end{figure*}

\noindent\textbf{Effect of anonymization on overhead:} In Figure \ref{Figure:solOne_overhead_level}, we present the time, CPU usage, and memory usage overhead for the execution of computations anonymized through the \solOne mode for different anonymization levels in a normalized form. Specifically, we normalize the required time to execute each anonymized computation by the required time to complete the same computation without anonymization. In the same manner, we also normalize the CPU and memory usage overhead. As Figure \ref{Figure:solOne_overhead_level} indicates, all three types of overhead show the same trend. The overhead to execute a computation increases as the anonymization level increases. This is due to the fact that a higher level of anonymization increases the complexity of the overall anonymization process (\eg  more ``fake'' nodes are added to computation graphs, padding of inputs and outputs becomes more extensive).

%The overhead come from the addition of ``fake'' nodes, removing the padding of the input, adding padding to the output, etc. and, since a higher order anonymization level means more fake nodes and padding added by \solOne mode to the original computation which, subsequently, increases the computation overheads.  

\noindent\textbf{Impact of anonymizing different features:} In Table \ref{tab:impact}, we present results on how anonymizing different computation features can impede the attack model's ability to identify computations. Our results demonstrate that adding padding only to inputs or outputs or even both is unable to reduce the attack model's effectiveness in a substantial manner. Nevertheless, anonymizing the completion time of computations by adding ``fake'' nodes reduces the accuracy of the attack model substantially as the anonymization level increases. Combining input and output padding and completion time anonymization results in the highest reduction of the attack model's accuracy.

%then we can achieve further anonymization.      


\begin{figure}[!t]
%\vspace{-0.2cm}
 \centering
 \includegraphics[width=1\columnwidth]{figs/solOne_overhead_level.pdf}
 \vspace{-0.5cm}
 \caption{Normalized overheads of \solOne for different anonymization levels} 
 \label{Figure:solOne_overhead_level}
 \vspace{-0.2cm}
\end{figure}


%\newline
%\textcolor{red}{Present results about the offline mode for both datasets. Present the following figures: 1. accuracy (y axis) for synthetic dataset for different machine learning models and for different levels of anonymization (x-axis, bar plots), 2. accuracy (y axis) for alibaba dataset for different machine learning models and for different levels of anonymization (x-axis, bar plots), 3. a table listing the accuracy for different cases (padded inputs, without process time, with only process time, etc.) for one machine learning model and then we can say that other models follow the same result trends, 4. time overhead for different levels of anonymization (box plots with average and standard deviation)}

\begin{table*}%
%\begin{minipage}{.25\linewidth}
\caption{Impact of anonymizing different features on attack model accuracy}
%\vspace{0.15cm}
\label{tab:impact}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{\begin{tabular}[c]{@{}c@{}}Anonymization\\ level\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Only input\\ padding\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Only output\\ padding\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Both input and\\ output padding\end{tabular}} & 
\textbf{\begin{tabular}[c]{@{}c@{}}Only completion\\ time anonymization\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}All features\\ anonymization\end{tabular}} \\ \hline
1 & 99.1 & 99.1 & 99.0 & 95.0 & 91.7                       \\ \hline
2 & 99.0 & 98.6 & 98.8 & 87.0 & 83.3   \\ \hline
3 & 99.1 & 97.5 & 98.5 & 77.0 & 75.4  \\ \hline
4 & 98.9 & 94.5 & 96.2 & 73.0 & 68.0   \\ \hline
5 & 99.1 & 91.2 & 95.2 & 67.0 & 57.9  \\ \hline

\end{tabular}
%\end{minipage}
\end{table*}


\begin{table}%
%\begin{minipage}{.25\linewidth}
\caption{Required time to anonymize a graph using \solOne mode}
%\vspace{0.15cm}
\label{tab:solOne_conversation_time}
\centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{\begin{tabular}[c]{@{}c@{}}Anonymization\\ level\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Required time\\ to anonymize (ms) \end{tabular}}  \\ \hline
1 &  7  \\ \hline
2 &  14  \\ \hline
3 &  25 \\ \hline
4 &  34  \\ \hline
5 &  40  \\ \hline

\end{tabular}
%\end{minipage}
\end{table}

\noindent\textbf{Required time to anonymize a computation graph:} Table \ref{tab:solOne_conversation_time} shows the required time to anonymize a graph on the fly using the \solOne mode (step 3a in Figure \ref{Figure:workflow} of our design) for different anonymization levels. Our results indicate that the required time increases as the anonymization level increases. For greater anonymization levels, the \solOne mode needs to introduce more ``randomness'' to computations which, subsequently, increases the anonymization time. Overall, our results show that the \solOne mode needs less than 40ms to anonymize a computation. In cases of delay-sensitive and highly private computations (which may require a greater anonymization level), computations can be anonymized in advance (pre-anonymized) as we discussed in Section~\ref{subsec:solone}. This amortizes the overall cost and eliminates the need to conduct computation anonymization on the fly.

\begin{comment}
\begin{itemize}
    \item how the overhead changes with the anonymization level
    \item how the accuracy changes with the anonymization level
    \item maximum level of anonymization... after a certain level, there should be no effect of increasing the level.
\end{itemize}
\end{comment}


\subsubsection{\mix mode}
%\newline
\noindent\textbf{\newline\newline Effect of anonymization on accuracy:} Figure \ref{figure:mixing_acc_batch} shows how the accuracy of different attack models is impacted as the number of computations that are shuffled together (\ie mixing batch size) varies for the \mix mode. Similar to the \solOne mode, as the batch size increases, the accuracy of all models for all three datasets decreases, since a higher batch size results in mixing more computations, thus making it harder for attackers to identify the computations being mixed. Overall, with the \mix mode, we are able to reduce the accuracy of the attack models by up to 50\%.  




\begin{figure*}[!th]
\vspace{-0.1cm}
\captionsetup[subfigure]{aboveskip=-0.00000000000000001pt,belowskip=-0.00000000000000001pt}
	\centering
	\begin{subfigure}{0.3\textwidth}
		\centering
		\includegraphics[scale=0.22]{figs/mixing_syn_acc_batch.pdf}
		\caption{Synthetic dataset.}
		\label{Figure:mixing_syn_acc}
	\end{subfigure} \hfil
	%\vspace{0.2cm}
	\begin{subfigure}{0.3\textwidth}
	    \centering
	    \includegraphics[scale=0.22]{figs/mixing_ml_acc_batch.pdf}
	    \caption{ML/AI dataset}
	    \label{Figure:mixing_ml_acc}
	\end{subfigure}\hfil
	\begin{subfigure}{0.3\textwidth}
	    \centering
	    \includegraphics[scale=0.22]{figs/mixing_alibaba_acc_batch.pdf}
	    \caption{Alibaba cloud dataset.}
	    \label{Figure:mixing_alibaba_acc}
	\end{subfigure}\hfil
	\vspace{-0.3cm}
	\caption{Identification accuracy of different attack models for different batch sizes using \mix mode.}
	\label{figure:mixing_acc_batch}
	\vspace{-0.2cm}
\end{figure*}

\noindent\textbf{Effect of anonymization on overhead:} In Figure \ref{Figure:mixing_overhead}, we present the overhead results introduced by mixing computations for different batch sizes. A mixing batch size equal to one indicates that computations are executed without anonymization. As a result, there is no additional overhead in this case. Both the time and CPU overheads show the same trend and increase as the mixing batch size increases. The time overhead is due to the execution of multiple computation graphs in a serialized manner (as shown in Figure \ref{Figure:mix}), whereas the CPU overhead is due to context switching among the nodes of different computation graphs.

Unlike the \solOne mode, the \mix mode does not add ``fake nodes'' to computation graphs or padding to inputs and outputs in order to anonymize computations. Because of that, there is no extra memory overhead introduced by the \mix mode. That is why the memory usage remains stable as the mixing batch size increases.

\begin{figure}[!t]
%\vspace{-0.2cm}
 \centering
 \includegraphics[width=1\columnwidth]{figs/mixing_overhead.pdf}
 \vspace{-0.5cm}
 \caption{Normalized overheads of \mix for different batch sizes} 
 \label{Figure:mixing_overhead}
 \vspace{-0.2cm}
\end{figure}


\noindent\textbf{Required time to anonymize a graph:} In Table \ref{tab:mix_conversation_time}, we present the time required to anonymize a graph using the \mix mode for different mixing batch sizes. Unlike the \solOne mode, the anonymization time is in the few microsecond ranges since the \mix mode only needs to select which node of which computation graph will be executed next instead of trying to conceal the features of each computation graph. 

\begin{table}%
%\begin{minipage}{.25\linewidth}
\caption{Required time to anonymize a graph using \mix mode}
%\vspace{0.15cm}
\label{tab:mix_conversation_time}
\centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{\begin{tabular}[c]{@{}c@{}}Mixing batch\\ size\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Required time\\ to anonymize (ms) \end{tabular}}  \\ \hline
2 &  0.009  \\ \hline
3 &  0.011 \\ \hline
4 &  0.019 \\ \hline
5 &  0.020  \\ \hline

\end{tabular}
%\end{minipage}
\end{table}




\begin{figure*}[!th]
\vspace{-0.1cm}
\captionsetup[subfigure]{aboveskip=-0.00000000000000001pt,belowskip=-0.00000000000000001pt}
	\centering
	\begin{subfigure}{0.3\textwidth}
		\centering
		\includegraphics[scale=0.22]{figs/mixing_parallel_syn_acc_batch.pdf}
		\caption{Synthetic dataset.}
		\label{Figure:mixing_parallel_syn_acc}
	\end{subfigure} \hfil
	%\vspace{0.2cm}
	\begin{subfigure}{0.3\textwidth}
	    \centering
	    \includegraphics[scale=0.22]{figs/mixing_parallel_ml_acc_batch.pdf}
	    \caption{ML/AI dataset}
	    \label{Figure:mixing_parallel_ml_acc}
	\end{subfigure}\hfil
	\begin{subfigure}{0.3\textwidth}
	    \centering
	    \includegraphics[scale=0.22]{figs/mixing_parallel_alibaba_acc_batch.pdf}
	    \caption{Alibaba cloud dataset.}
	    \label{Figure:mixing_parallel_alibaba_acc}
	\end{subfigure}\hfil
	\vspace{-0.3cm}
	\caption{Identification accuracy of different attack models for different batch sizes using parallel \mix mode.}
	\label{figure:mixing_parallel_acc_batch}
	\vspace{-0.2cm}
\end{figure*}


\noindent\textbf{\newline\newline Effect of anonymization on accuracy for parallel \mix mode:} The results presented in Figure \ref{figure:mixing_parallel_acc_batch} show how the accuracy of the attack models changes when computation graphs are mixed together and run in parallel. Similar to the serialized \mix mode, the accuracy of the attack models drops for all three datasets as the mixing batch size increases. In most cases, the parallel \mix mode has been able to impair the ability to identify computations slightly more as compared to the serialized \mix mode. Because, in the parallel mode, the required computation time of a graph can be either less or more than the actual computation time of the graph since there are multiple threads and the nodes of a graph can be executed by one or more threads. Where, in serialized mode, the required computation time is always more than the actual computation time. Because of this randomness of computation times, the parallel \mix mode is relatively more effective to anonymize computation graphs. 


\begin{comment}


\begin{figure}[!t]
%\vspace{-0.2cm}
 \centering
 \includegraphics[width=1\columnwidth]{figs/mixing_overhead_parallel.pdf}
 \vspace{-0.5cm}
 \caption{Normalized overheads of parallel \mix for different batch sizes} 
 \label{Figure:mixing_parallel_overhead}
 \vspace{-0.2cm}
\end{figure}
\end{comment}



\begin{table}%
%\begin{minipage}{.25\linewidth}
\caption{Required time to anonymize a graph using \mix mode}
%\vspace{0.15cm}
\label{tab:mix_parallel_conversation_time}
\centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{\begin{tabular}[c]{@{}c@{}}Mixing batch\\ size\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Required time to \\ anonymize using parallel \\ \mix mode (ms) \end{tabular}}  \\ \hline
2 &  0.0008  \\ \hline
3 &  0.0011 \\ \hline
4 &  0.0014 \\ \hline
5 &  0.0016  \\ \hline

\end{tabular}
%\end{minipage}
\end{table}


\noindent\textbf{Required time to anonymize graphs using parallel \mix mode:} The required time to mix different numbers of graphs are in the magnitude of microseconds as shown in Table \ref{tab:mix_parallel_conversation_time}. The required anonymization time is less than the \solOne mode and the serialized \mix mode. Because there is no need to anonymize each graph individually as the \solOne mode does, and each thread selects which node it will execute next, unlike the serialized \mix mode where there is only a single thread to perform the node selection.  




\subsubsection{\hybrid mode}


\begin{figure*}[!th]
\vspace{-0.1cm}
\captionsetup[subfigure]{aboveskip=-0.00000000000000001pt,belowskip=-0.00000000000000001pt}
	\centering
	\begin{subfigure}{0.3\textwidth}
		\centering
		\includegraphics[scale=0.22]{figs/hybrid_syn_acc_batch.pdf}
		\caption{Synthetic dataset.}
		\label{Figure:hybrid_syn_acc}
	\end{subfigure} \hfil
	%\vspace{0.2cm}
	\begin{subfigure}{0.3\textwidth}
	    \centering
	    \includegraphics[scale=0.22]{figs/hybrid_ml_acc_batch.pdf}
	    \caption{ML/AI dataset}
	    \label{Figure:hybrid_ml_acc}
	\end{subfigure}\hfil
	\begin{subfigure}{0.3\textwidth}
	    \centering
	    \includegraphics[scale=0.22]{figs/hybrid_alibaba_acc_batch.pdf}
	    \caption{Alibaba cloud dataset.}
	    \label{Figure:hybrid_alibaba_acc}
	\end{subfigure}\hfil
	\vspace{-0.3cm}
	\caption{Identification accuracy of different attack models for different batch sizes using \hybrid mode.}
	\label{figure:hybrid_acc_batch}
	\vspace{-0.2cm}
\end{figure*}

\noindent\textbf{\newline\newline Effect of anonymization on accuracy:} Our experiment results demonstrate the similar trend for all possible combinations of anonymization levels and both the serialized and parallel \mix modes. Because of space constraint, we do not present all results. For the evaluation of \hybrid mode, we present the results of \hybrid mode in Figure \ref{figure:hybrid_acc_batch}, where we first anonymize graphs using the \solOne mode (anonymization level = 3), and then these anonymized are mixed together using the parallel \mix mode. As Figure \ref{figure:hybrid_acc_batch} shows that the \hybrid mode is more effective in impairing the computation identification ability of the attack model as compared to the \solOne mode for the particular anonymization level and for different batch sizes of the \mix mode individually.  

\noindent\textbf{Effect of anonymization on overhead and required time to anonymize graphs:} Since the \hybrid mode is the combination of the \solOne mode and the \mix mode, both the required time to anonymize a computation graph is the summation of individual required time to anonymize the graph using the \solOne and \mix modes. Similarly, the overhead to execute the graph is the combined overhead of both modes.  


\subsubsection{Performance of adaptive attack model}








\begin{figure*}[!th]
\vspace{-0.1cm}
\captionsetup[subfigure]{aboveskip=-0.00000000000000001pt,belowskip=-0.00000000000000001pt}
	\centering
	\begin{subfigure}{0.3\textwidth}
		\centering
		\includegraphics[scale=0.22]{figs/adaptive_syn_acc.pdf}
		\caption{Synthetic dataset.}
		\label{Figure:adaptive_syn_acc}
	\end{subfigure} \hfil
	%\vspace{0.2cm}
	\begin{subfigure}{0.3\textwidth}
	    \centering
	    \includegraphics[scale=0.22]{figs/adaptive_ml_acc.pdf}
	    \caption{ML/AI dataset}
	    \label{Figure:adaptive_ml_acc}
	\end{subfigure}\hfil
	\begin{subfigure}{0.3\textwidth}
	    \centering
	    \includegraphics[scale=0.22]{figs/adaptive_alibaba_acc.pdf}
	    \caption{Alibaba cloud dataset.}
	    \label{Figure:adaptive_alibaba_acc}
	\end{subfigure}\hfil
	\vspace{-0.3cm}
	\caption{ Performance of different adaptive attack models.}
	\label{figure:adaptive_acc}
	\vspace{-0.2cm}
\end{figure*}



For the evaluation of the adaptive attack model (as described in Section \ref{sec:threat}), we run experiments with the \solOne mode, the \mix mode, and the hybrid mode for all three datasets. For anonymization level 5 and batch size 5, as Figure \ref{figure:adaptive_acc} shows, the accuracy of different attack models remains within the range of 44\%-57\%, even after re-training the attack models over time.    

%\textcolor{red}{Present results about the mix-n-match mode for both datasets. Present the following figures: 1. accuracy (y axis) for synthetic dataset for different machine learning models and for different sizes of mix-n-match batches (x-axis, bar plots), 2. accuracy (y axis) for alibaba dataset for different machine learning models and for different levels of anonymization (x-axis, bar plots), 4. time overhead for different batch sizes (box plots with average and standard deviation)}

%-----


%Our dataset contains the name of the graph, its input and output size, the numbers of inputs and outputs needed by the graph along with the time it takes for the graph to complete execution from the moment it was called by the user. To conduct an evaluation on the concept of fake nodes on computational graphs we created our own synthetic dataset that includes the result of annonymizing ten computational graphs with identical pairs. The identical pairs are graphs that look the same but their nodes conduct completely different operations. We used simple processes in the nodes that included sorting, encryption, decryption, compression and solving simple mathematical equation solving. 



%We assume that the attacker has privilege in the server and can gain the necessary information required to train a machine learning model that can guess the graph that was requested by the user. As we designed 10 different graphs, the first step is to prove if a machine learning model can determine the particular graph being executed from the limited set of information available. To create the dataset we ran each graph with different inputs and noted down the information from the execution of each graph. Following this method we collected 100 execution results from each graph. Now, with the available result we train a machine learning model with K-Means [Refer KMeans] clustering algorithm to determine a graph from its execution information. Using a train\_test\_split of 80 and 20 percent on the entire dataset containing 1000 graph execution we generate a detection accuracy of 99\%. 


%\noindent\textbf{Data Extraction Alibaba Cluster Trace Dataset: } For the cluster trace dataset, we do not have to run the computations for each graph and add the data to the dataset. Instead, the dataset already has the information of a particular task, its sub task, the start and end time, memory used and cpus needed for the task. We choose the batch task table because it contains the minimum amount of information needed to deduce the task type. The dataset is very large and contains lots of extreme values especially concerning time. The data available for task type 2 and 7 are very limited and so we continue by dropping them from the type list. Again, we have 10 sets of graphs that have to undergo anonymization. Before we apply our methods, we test the detection accuracy for the remaining task types using the K-Means Clustering and the same split size of 20\% as before to get 86.5\%.

%\subsection{Fake Nodes on Synthetic Dataset}
%Considering the high level of graph detection accuracy we move forward to attach the same process for computation graph execution for generating the dataset containing the fake nodes. We allow the users to choose the number of fake nodes for their execution, by altering a single variable for anonymization level. We start collecting data from level 1 and continue until level 5. With the results from all the computation graph execution we have a total of 6 data tables for six levels of anonymization starting from 0 where no fake nodes were added. Level 0 is meant to perform similarly to a process without any mechanism for adding fake nodes. We keep the data as a pivot to compare against anonymized level data for testing.  This way, we clarified how much each level of anonymization affected the detection accuracy for each computation graph. We verified our results using multiple machine learning algorithms like SVM and a Basic Neural Network model from Keras [Refer Model]  and CNN [Refer Model]. \newline
%[table of results] \newline
%The table above shows our initial results from using the different Machine Learning algorithms with the Level 0 data for training and testing with the different levels of anonymization. From the results we can conclude that just by causing a change in execution time due to fake computations we can reduce the detection accuracy.\newline
%[graph of anonymization against time]

%\subsection{Mix \& Match on Synthetic Dataset}
%We applied our second approach for computation anonymization on the same 10 graphs used in our first method. This time instead of creating a fake node we create a larger graph that contains the nodes of multiple graphs. To avoid long execution times we limited the number of graphs for the larger graph and took the similar graphs together to make three larger graphs from the initial 10. We applied our process and it provided even better results than fake nodes 56\% from KNN[R] and 54\% from the Neural Network[R] approach. However, following this approach will lead to an increased execution time for some computations as they mostly take the time of the longest executing node in a graph. To avoid this problem we generated a weight mechanism that puts a weight on computations that require less time and resources to complete. We were able to stop the instances using the weights but during some executions the longest resource consuming node still gets executed even though the probability is very low. Following the weighted mix and match approach we get a detection accuracy of 72\% from KNN[Refer KNN] and 70\% from Neural Networking [Refer NN] algorithm.

%\subsection{Fake Nodes on Alibaba Cluster Trace Dataset}
%\subsection{Mix \& Match on Alibaba Cluster Trace Dataset}

%\noindent\textbf{Alibaba Dataset: }

%\noindent\textbf{Fake Nodes on Alibaba Dataset: }
\begin{comment}


\begin{itemize}
    \item \textcolor{red}{We need some real-world graphs and create a dataset for these graphs. Also, we need to describe the experiment setup and how we collect the data(such as how the attack identify the size/number of  input/output for a real-world graph). Only synthetic graphs and dataset will not help. I don't think the reviewers will be satisfied.}
\end{itemize}

\end{comment}

